Could GRB 060614 and its presumed host galaxy be a chance superposition?

The lack of an observed supernova associated with GRB 060614 appears to require a new paradigm for the formation of (a subset of) long-duration GRBs. This requirement is based on the presumed low redshift of the burst, which was inferred from the spatial coincidence of the afterglow with a z=0.125 galaxy. We explore the possibility that this low-redshift galaxy is a chance superposition along the line of sight to GRB 060614. We examine the galaxy distribution of the field of GRB 060614 and find that the probability of a chance association with a galaxy at least as bright as the putative host is only ~ 0.5 - 1.9%. However, for the current ensemble of ~180 Swift GRBs it is likely that several such coincidences have occurred, and given the "non-standard" nature of GRB 060614 it is not implausible that this is one such occurrence. Thus the conclusion that GRB 060614 requires a revision to the formation paradigm for long-duration GRBs should be approached with caution.

==> response <==
 Dear Dr. Sneden,

 Enclosed please find a revised version of our paper "Could GRB 060614
 and its presumed host galaxy be a chance superposition?".  We 
 appreciate the referee's insightful comments, which have helped
 us to improve this Letter.  Below, we detail our response to the referee's
 specific comments.  Additionally, we received other outside comments
 on our paper, many of which were similar in nature to those made
 by our referee.  We have also made a few minor changes in response
 to those critiques, including specifically addressing the issue 
 of GRB 060505, which has also been suggested to be a low-redshift
 GRB without an observed SN.  

 Best wishes,
 Bethany Cobb, Charles Bailyn, Pieter van Dokkum, Priya Natarajan

REFEREE: 
>      Although I think that this is an important paper I find it to be
> somewhat rushed, and it does not treat the probability argument with
> enough rigour to make a strong statement about the probability of a
> chance alignment.  First, the authors assume that all of the galaxies
> that are detected by SExtractor are at a smaller redshift than the
> burst.  However, some fraction of the galaxies will be located at
> redshifts significantly greater than 0.125.  The correct way to state
> the probability is to say that there is a probability of X that the
> burst will occur within Y arcsec of a foreground galaxy with a
> redshift of <=Z where Z is <= the redshift of the burst.  All galaxies
> with a redshift greater than the (unknown) redshift of the burst
> should be excluded.  This is not trivial to do in a statistical sense,
> but it is necessary to obtain a meaningful result.  Studies of the
> redshift distribution of field galaxies suggest that a significant
> fraction of galaxies with I ~= 22 are at redshifts > 0.2, so this
> could be introducing a large error into the paper's result.
RESPONSE:
This is a reasonable worry, and to deal with this issue we have now
explicitly taken galaxy redshift distribution into account in 
section 3.

REFEREE:
>      Second, the authors do not consider the total chain of events
> that go into the association of a burst with a galaxy when they arrive
> at their 0.02 probability.  For example, the lack of absorption
> systems with z > 0.125 in the burst's spectrum should be taken into
> account since this suggests that the burst occurred at low redshift.
> What is the probability that that no absorption systems will be seen
> in the spectrum of a burst with z less than some arbitrary value in a
> random direction in the field of view.  Another example is that the
> authors do not model the process by which a supernova component to the
> light curve is detected.  SNe have only been identified for a small
> fraction of bursts.  The degeneracy between high redshift and dust
> absorption means that in general the lack of a supernova bump is not
> taken to indicate that the burst had z >~ 1.  This should be
> considered in computing the probability.  In addition, the association
> of GRB 060614 with the putative host galaxy draws on the knowledge of
> the spectral energy distribution of the burst (which can be
> constructed using public Swift data).  My quick-and-dirty XSpec
> modelling suggests z = 0.24, with a large uncertainty.  Therefore, the
> probability of the spectral energy distribution mimicing a
> low-redshift burst (which was one of the bases of the association
> between the burst and the galaxy) needs to be included in the
> calculation.
RESPONSE:
While we acknowledge that the lack of any absorption features
in the afterglow spectrum may argue for a low-redshift origin
for this burst, we cannot comment more than generally on this issue because
we do not have access to the spectral data to examine more fully (since the
afterglow spectrum has not been published in the literature).

REFEREE:
>      Computing the the probability of a chance alignment without
> resorting to a priori reasoning is not easy and probably requires a
> detailed study of a large sample of randomly selected, well-localized
> gamma-ray bursts.  This sort of study is well beyond the scope of an
> ApJ Letter.  I urge the authors to undertake such a study as it will
> be a significant contribution to the field of gamma-ray burst study.
RESPONSE:
In fact, such a paper is currently in preparation.  GRB 060614
needed to be rapidly addressed on an individual basis, however,
because of the current great interest it has sparked in the literature.

REFEREE:
>      Despite my concerns with the methodology I recommend that this
> paper be published as an ApJ Letter with one caveat.  The probability
> that the authors derive is actually an upper limit on the true
> probability of a chance alignment.  This should be make clear in the
> text of the paper, and in the abstract.  
RESPONSE:
Given our additional calculation, which takes the redshift distribution into account,
we believe that our revised numbers represent the true range of probability, rather
than just an upper limit.  The assumptions that go into the calculation
of these numbers have been laid out in the text.
 
REFEREE:
> 1) Introduction, Paragraph 1, Line 3:
> 
>    The Hjorth et al. (2003) paper should be referenced since the
>    discovery of the supernova component was made independently by both
>    the Stanek and Hjorth groups.
RESPONSE:
This reference has been added.
 
REFEREE:
> 2) Introduction, Paragraph 5, Point 2:
> 
>    It would be useful to the reader to point out that SNe Ib/c have a
>    wide range of peak magnitudes, so it is not unreasonable that SNe
>    associated with GRBs would also exhibit a wide range of peak
>    magnitudes.
RESPONSE:
We have added the following sentence to make this point clear:
	"While local non-GRB Type Ibc SNe do span a larger range of +/- ~2 
	magnitudes from the peak of SN 1998bw (Richardson et al. 2006), even
	the dimmest known Ibc SN should have been detectable in the absence 
	of strong reddening."

REFEREE:
> 3) Data, Paragraph 1:
> 
>    I suggest that the authors present a Figure showing their
>    photometry.
RESPONSE:
A new Figure 1 has been added to show our photometry.  We have also added
to this graph various expected curves for a SN event in the galaxy
to emphasize the absence of such an event in our data.
    
REFEREE:
> 4) Discussion, Paragraph 1:
> 
>    The probability of a chance alignment in the Swift sample depends
>    strongly on the positional accuracy of the Swift bursts.  This
>    varies greatly from burst to burst.  Only about 33% of the Swift
>    bursts have the sub-arcsecond precision needed to make a reasonable
>    assignment of a host galaxy.  This reduces the number of useful
>    bursts from ~180 to ~60, which implies that there has only been one
>    chance alignment so far.
RESPONSE:
This has now been addressed as follow:
	"The strongest host galaxy claims can only be made for GRBs with
	detected optical afterglows.  Of the $\sim80$ optical afterglows detected following
	Swift bursts, the detection of no chance overlaps would not be unexpected
	at a probability of 22\% to 67\%."

REFEREE:
> 5) Table 1:
> 
>    The authors should specify whether the "Observation UT date" refers
>    to the start of the observation, the middle, or some other time.
>    The authors should also state the significance level of the upper
>    limits.
RESPONSE:
These issues have now been specified in the table captions as follows:
	"Mid-exposure time of images in days after the burst trigger, which occurred 
	at 2006 June 14, 12:43:48 UT."
	"These values have not been corrected for Galactic extinction. 3\sigma limiting 
	magnitudes are reported for observations in which the galaxy is not significantly detected."


